Airdrops and Privacy: A Case Study in Cross-Blockchain Analysis

Airdrops are a popular method of distributing cryptocurrencies and tokens. While often considered risk-free from the point of view of recipients, their impact on privacy is easily overlooked. We examine the Clam airdrop of 2014, a forerunner to many of today's airdrops, that distributed a new cryptocurrency to every address with a non-dust balance on the Bitcoin, Litecoin and Dogecoin blockchains. Specifically, we use address clustering to try to construct the one-to-many mappings from entities to addresses on the blockchains, individually and in combination. We show that the sharing of addresses between the blockchains is a privacy risk. We identify instances where an entity has disclosed information about their address ownership on the Bitcoin, Litecoin and Dogecoin blockchains, exclusively via their activity on the Clam blockchain.

==> Makefile <==
TEXFILES = main.tex tex/abstract.tex tex/introduction.tex \
  tex/related-work.tex tex/four-blockchains.tex tex/cluster-analysis.tex \
  tex/tx-analysis.tex tex/single-blockchain-impact.tex \
  tex/multi-blockchain-impact.tex tex/conclusion.tex \
  tex/appendices.tex
IMGFILES = img/cluster-analysis/bitcoin/bitcoin.png \
  img/cluster-analysis/clam/clam.png \
  img/cluster-analysis/dogecoin/dogecoin.png \
  img/cluster-analysis/litecoin/litecoin.png \
  img/cluster-analysis/bitlitedoge/bitlitedoge.png \
  img/cluster-analysis/bitlitedogeclam/bitlitedogeclam.png \
  img/combination-diff/combination-diff.png \
  img/co-cluster-graph/bitcoin-clam/bitcoin-clam.png \
  img/tx-analysis/bitcoin/bitcoin.png \
  img/tx-analysis/clam/clam.png \
  img/tx-analysis/dogecoin/dogecoin.png \
  img/tx-analysis/litecoin/litecoin.png \
  img/tx-analysis/bitlitedoge/bitlitedoge-annotated.png \
  img/tx-analysis/bitlitedogeclam/bitlitedogeclam-annotated.png \
  img/clam-address-sharing/main.pdf \
  img/co-cluster-graph/main.pdf \
  img/clustering-improvements/main.pdf
BIBFILES = bib/main.bib

.PHONY: all clean

all: main.pdf

main.pdf: $(TEXFILES) $(IMGFILES) $(BIBFILES) 
	latexmk -pdf -use-make $<

clean:
	latexmk -CA


==> img/cluster-analysis/Makefile <==
SUBDIRS := $(wildcard */.)

.PHONY: all $(SUBDIRS)

all: $(SUBDIRS)

$(SUBDIRS):
	$(MAKE) -C $@

clean:
	for d in $(SUBDIRS); do \
		$(MAKE) -C $$d clean; \
	done


==> img/tx-analysis/Makefile <==
SUBDIRS := $(wildcard */.)

.PHONY: all $(SUBDIRS)

all: $(SUBDIRS)

$(SUBDIRS):
	$(MAKE) -C $@

clean:
	for d in $(SUBDIRS); do \
		$(MAKE) -C $$d clean; \
	done

